Turning Tables: Generating Examples from Semi-structured Tables for Endowing Language Models with Reasoning Skills

Models pre-trained with a language modeling objective possess ample world knowledge and language skills, but are known to struggle in tasks that require reasoning. In this work, we propose to leverage semi-structured tables, and automatically generate at scale question-paragraph pairs, where answering the question requires reasoning over multiple facts in the paragraph. We add a pre-training step over this synthetic data, which includes examples that require 16 different reasoning skills such as number comparison, conjunction, and fact composition. To improve data efficiency, we propose sampling strategies that focus training on reasoning skills the model is currently lacking. We evaluate our approach on three reading comprehension datasets that are focused on reasoning, and show that our model, PReasM, substantially outperforms T5, a popular pre-trained encoder-decoder model. Moreover, sampling examples based on current model errors leads to faster training and higher overall performance.

==> 01_intro_old.tex <==
\section{Introduction}

Large pre-trained language models, such as T5 and GPT-3 have been shown to capture a wide variety of linguistic skills, which enables them to reach new heights on natural language processing tasks such as reading comprehension and question answering. During the process of pre-training, these models seem to acquire large amounts of factual knowledge \citep{roberts2020knowledge} and commonsense reasoning.

However, recent work suggests that some reasoning skills are not acquired from pre-training. For example:
 \citep{wallace2019nlp} show that BERT poorly captures numerical skills, such as finding the maximal value in a list,
\citep{hidey-etal-2020-deseption} suggest that LM struggles with temporal reasoning, such as date comparisons and ordering of events, \citep{talmor2020olmpics} argue that different models acquire different skills from pre-training, and discuss to what extent pre-trained models capture symbolic reasoning skills such as conjunction and composition.

To handle these problems, recent work has suggested adding reasoning components to existing architectures \citep{ran2019numnet}, \citep{hidey-etal-2020-deseption} and adding an intermediate training step between pre-training and fine-tuning which is more similar to the downstream tasks. For example, masking spans that are relevant for temporal skills, or automatic generation of numeric synthetic data \citep{geva2020injecting}, \citep{moosavi2021learning}.
 
In this work, we propose that structured data from the web can be used to introduce a new self-supervised training task that is reach in reasoning skills. More specifically, large amounts of information is stored in Wikipedia tables.  By flattening tables to textual phrases, we can artificially generate large numbers of question-answer pairs that require complex reasoning, such as numeric, temporal, or logical skills. Previous work had leveraged semi-structured tables as a mean to improve performance on tabular QA \cite{eisenschlos2020understanding}. As far as we are aware, we are the first to propose leveraging semi-structured data to introduce a new sequence-to-sequence task, and empirically show that this improves performance on reading comprehension tasks.

We first flatten a table to a set of textual facts, which can contain textual, numeric or temporal values. We then utilize hand-made templates to generate a large and diverse set of question-answer pairs, alongside contexts of facts that are necessary to correctly answer the question. We make sure that the generated questions require reasoning skills such as: counting, comparison, conjunction, quantifiers, comparison, superlatives, arithmetic, and temporal skills. Overall, we generate XXXX questions, about XXXX skills from XXXX tables. 

To enhance existing models with additional skills, we introduce a second step of training between pre-training and fine-tuning, named continuous pre-training (CPT). During CPT, the reasoning intensive tasks are learnt alongside the original MLM objective, in order to avoid catastrophic forgetting. We show that our reasoning enhanced model maintains performance on both the original MLM objective and on downstream tasks.  Contrary to previous works, we rely solely on the distribution of the values in the tables, and do not make any changes to a standard encoder-decoder Transformer architecture.

Since the number of generated examples for every task is extremely large, and the performance of the model on every task is unknown before CPT, we experiment with two dynamic sampling algorithms. In the first approach, we sample from each task in linear accordance with the errors for each task, such that tasks with lower performance are over-sampled. In the second approach, we dynamically calculate the improvement for each task in a specific time window, such that tasks that are currently improving are over-sampled. We show that both methods outperform a naive uniform approach. 

Additionally, we show that we can also utilize our generated data to enhance our REM models with explainablity skills. In order to enhance explainability skills we add a new task to CPT, in which the model has to generate the reasoning skill required to answer a question. We find that a model which is fine-tuned a downstream task is still able to generate required skills far better than a random baseline (xxxx vs xxxx), while not receiving any explicit supervision on the reasoning skills in the downstream task.  We show that the explainable model is even able to generalize to templates that were not seen during CPT.

Finally, we present base and large sized reasoning enhanced models: REM-Base and REM-Large. We evaluate our REM models on three datasets that require complex reasoning skills: MMQA, IIRC and Drop. Our REM models significantly outperform the original T5 models on all three datasets. Our REM-Large model achieves new state of the art results in MMQA, and on the IIRC oracle setting. 

 We provide an analysis that shows that the improvement in performance is due to acquired reasoning skills in tasks such as: conjunction, counting, comparison, superlatives, arithmetics and temporal reasoning. We show that the improvement on specific  question types, such as IIRC value quesitons, MMQA comparison questions, and Drop arithmetic questions is especially significant, XXXX, XXXX, XXXX points respectively. Additionally, we show that our models are scalable, such that significant improvements are seen both for base and large size models and are able to generalize to new question templates that were not seen during CPT. 

To summarize, our key contributions are:

\begin{itemize}
  \item Introduce a new method to generate a large amount of reasoning rich self-supervised data by leveraging structured data from the web
  \item Introduce a continuous pre-training framework for efficiently enhancing pre-trained models with reasoning skills while preserving performance on the original pre-training task
  \item Show that our method can be used to enhance explainability in pre-trained LMs without any supervision on the downstream task
  \item Introduce two new models, REM-Base and REM-Large, which outperform the original T5-models on 3 reasoning intensive benchmarks
\end{itemize}


==> 02_problem_setup.tex <==
\section{Problem Setup}

% \begin{itemize}
% \item Why we propose tables
% \item Syn-To-Real, Structured-To-Unstructured
% \item overview of our framework
% \item definitions
% \item how we train our method: dynamic sampling + CPT
% \end{itemize}


Our goal is to train a RC model that given a question $q$ and textual context $c$ returns an answer $a$ (Fig.~\ref{fig:intro}), given a training set $D = \{(q_i, c_i, a_i\}_{i=1}^N$.
%\jb{suggestion: `Our goal is to train a model that given a question $q$ and textual context $c$ returns an answer $a$ (see Fig.~\ref{fig:intro}), given a training set $D = \{(q_i, c_i, a_i\}_{i=1}^N$}. 
We focus on questions that require reasoning over the context $c$, for example, composing two distinct facts.
%\jb{delete `complex', vague} reasoning \jb{add `operation'} over the context $c$, for example, composing two \jb{distinct} facts that appear in $c$. 
%Recent research \cite{wallace-etal-2019-nlp, geva-etal-2020-injecting, talmor2020olmpics, nie-etal-2020-adversarial, hidey-etal-2020-deseption} has shown that the reasoning skills of pre-trained language models (LMs) are partial, and acquiring them from the training set $D$ might be difficult when $D$ is small. 
To endow LMs with reasoning skills, we would like to automatically generate a large synthetic training set $D_\textit{syn} = \{(q_j, c_j, a_j)\}_{j=1}^{M}$ (where $M \gg N$) from semi-structured tables, before fine-tuning on a target dataset.

%\jb{Recent research} \jb{has shown} that pre-trained language models (LMs) \jb{make sure to define LM before} lack \jb{replace `are not equipped with' with 'lack'} reasoning skills from pre-training and that $D$ might be too small to learn those. Thus,  we would like to have an automatic process for generating a synthetic training set $D_{syn} = \{(q_i, c_i, a_i\}_{i=1}^N$.
%\jb{proposal: ... that the reasoning skills of pre-trained LMs are partial, and acquiring them from the training set $D$ might be difficult when $D$ is small. Thus, we would like to develop an automatic method for generating a large synthetic training set $D_\textit{syn} = \{(q_j, c_j, a_j\}_{j=1}^{M}$ that will improve the reasoning skills of a pre-trained LM (where $N \ll M$).}


%Our insight is that semi-structured tables provide a rich information source for automatically generating $D_{\textit{syn}}$.
%Tables can be crawled from the web at scale \cite{pasupat-liang-2015-compositional,herzig-etal-2020-tapas, eisenschlos-etal-2020-understanding, DBLP:journals/corr/abs-2104-00369} and provide information on a wide range of topics. Moreover, due to the semi-structured nature of tables, one can detect columns with numbers and dates, which facilitates automatic generation of examples that involve reasoning.

%Fig.~\ref{fig:overview} provides an overview of our approach. We generate $(q,c,a)$ triplets from tables such that to arrive at the answer $a$, one needs to reason over multiple textual facts from the context $c$, which  are generated from the table and are phrased using a pseudo-language (see Fig.~\ref{fig:intro}). Examples are generated using Example Generators (EGs), each corresponding to a different reasoning skill (\S\ref{sec:data_generation}).
%Since we can generate a very large number of examples, it is important to focus training on reasoning skills that the model lacks, and thus we use \emph{error-driven sampling} to construct training batches where most examples are from EGs that model fails on (\S\ref{sec:training}).
%Last, we fine-tune our model on downstream tasks that require reasoning. We show that training on synthetic examples substantially improves performance on three different reading comprehension datasets that require reasoning, and that error-driven sampling is beneficial (\S\ref{sec:experimental_setup}).


%Specifically, we generate $(q,c,a)$ triplets from tables such that to arrive at the answer $a$, one needs to reason over multiple facts from the context $c$ that are derived from the table and are phrased using a pseudo-language (see Fig.~\ref{fig:intro}).
%\jb{use the fig. Ori is preparing once it exists}

%\jb{multiple facts from the context $c$ that are derived from the table and are phrased using} a pseudo-language (PL) \jb{PL is usually programming language so not sure I am a fan of this acronym} textual context $c$ derived from the table \jb{delete the end of the sentence here. Also refer to the intro figure again}. 

%We argue \jb{Our insight is} that \jb{semi-structured} tables provide a good setup \jb{information source} to automatically generate \jb{for automatically generating} $D_{syn}$ \jb{$D_{\textit{syn}}$}, since they contain vast amounts of \numeric{}, \temporal{}, and \textual{} lexically diverse data in a semi-structured setup that enables easily generate questions and contexts using templates. More specifically, we generate $(q,c,a)$ triplets from tables such that to arrive at the answer $a$, one needs to reason over \jb{multiple facts from the context $c$ that are derived from the table and are phrased using} a pseudo-language (PL) \jb{PL is usually programming language so not sure I am a fan of this acronym} textual context $c$ derived from the table \jb{delete the end of the sentence here. Also refer to the intro figure again}. 
%\jb{I would put a full stop before ', since...' and the write something like: `Tables can be crawled from the web at scale (add refs) and provide information on a wide range of topics, which leads to high lexical diversity. Moreover, due to the semi-structured nature of tables, one can detect columns with numbers and dates, which enables automatic generation of questions and contexts using templates. Specifically, ...}

%In \S\ref{sec:data_generation}, we describe our example generation process. Since we can generate a very large number of examples for multiple reasoning skills, we can control the distribution of generated examples and focus training on skills that the model struggles with. In \S\ref{sec:training}, we describe our training procedure, including approaches for sampling examples such that the model improves more quickly on desired skills. Last, in \S\ref{sec:experimental_setup} we describe our experimental evaluation, where we show that training on synthetic examples substantially improves performance on three different reading comprehension datasets that require reasoning


%Since we automatically generate $D_{syn}$ from tables, we can tilt the distribution such that the reasoning the model has to perform in order to answer questions in $D_{syn}$ requires complex skills that may be different from the ones seen during pre-training. We now first describe the data generation procedure \S\ref{sec:data_generation}, how we train our model using this data \S\ref{sec:training} followed by experiments \S\ref{sec:experimental_setup}.
%\jb{Proposal: `in \S\ref{sec:data_generation}, we describe our process for generating questions from tables. Since we can generate a very large number of examples for every possible reasoning skill, we can control the distribution of generated examples and focus on skills that the model struggles with. In \S\ref{sec:training}, we describe our training procedure, including several approaches for sampling examples from the example generator. last, in \S\ref{sec:experimental_setup} we describe our experimental evaluation, where we show that training on synthetic examples substantially improves performance on three different question answering datasets that require reasoning.}

%\oy{see figure 1}. When one has to reason  since tables contain vast amounts of \temporal{}, \numeric{} and \textual{} information with high lexical and domain diversity.

%We think tables are good (see figure) and now describe in detail how we use tables to construct $D_{syn}$.


==> 07_analysis.tex <==
\section{Analysis}

%In this section, we provide additional analysis of our results. First, we focus on IIRC questions that require date difference reasoning to check generalization of our synthetic data $D_\textit{syn}$ to natural language and the effect of our error-driven sampling strategies. Then, we use a previous set of annotated questions \cite{Gupta2020Neural} from the DROP dataset to analyse which reasoning skills were injected to our \rem{} models.

\paragraph{Generalization to natural language}

\begin{table}
\centering
        \tiny
        \begin{tabular}{lcccc} \toprule
        
        \emph{Phrase} & \# & $D_\textit{syn}$ & \tfive{} & \rem{} \\ \midrule 
        \emph{how long...} & 59 & \cmark & 9.6 & \textbf{50.3}  \\ 
        \emph{how many years...} & 28 & \cmark & 10.7 & \textbf{57.1}  \\ 
        \emph{how many time...} & 4 &\cmark & 0.0 & \textbf{75.0}  \\ 
        \emph{how old...} & 76 &\xmark & 6.6 & \textbf{59.2}  \\ 
        \emph{what age...} & 13 &\xmark & 7.7 & \textbf{61.5} \\ \midrule 
        Other & 53 & & 20.1 & \textbf{33.3}  \\ 
        Total & 233 &  & 10.9 & \textbf{51.2}  \\ 
        \bottomrule 
         
        \end{tabular} 
\caption{F$_1$ on IIRC \emph{Value} questions with a breakdown to different date difference phrases. Phrases that are similar to those in $D_\textit{syn}$ are indicated.} 
\label{tab:analysis-generalization}
\end{table}

Many of the questions in IIRC require date difference reasoning. More specifically, more than $77.2\%$ of the \value{} questions in the development set include one of 5 date difference phrases: 3 of those are similar to phrases that are part of templates used by our date difference EG, while the other 2 were not seen before fine-tuning. Table~\ref{tab:analysis-generalization} presents the breakdown for our best \rem{-Large}/\tfive{-Large} IIRC$_\textrm{oracle}$ models to phrases that indicate date difference reasoning. We find that our \rem{} models are able to generalize extremely well to natural language questions that require similar to reasoning to $D_\textit{syn}$.

\paragraph{Effect of error-driven sampling}

In previous sections, we showed that our error-driven strategies lead to better performance on $D_\textit{syn}$ and IIRC$_\textrm{oracle}$ (see table~\ref{tab:rem-comparison} and fig~\ref{fig:syn-results}), and that many of the questions in IIRC require date difference reasoning. We now analyse whether improvements on $D_\textit{syn}$ due to error-driven sampling correlate with improvements over natural language questions that require date difference reasoning, as defined in the previous section. Fig.~\ref{fig:analysis-syn-to-real} shows that on large size models our uniform sampling strategy under-samples date difference questions by as much as about $40\%$ in comparison do our error-driven strategies, which corresponds with significantly worse performance of about $10$\fone{} on natural language questions.

\begin{figure}
  \includegraphics[width=1.0\columnwidth]{figures/syn-to-real 1.2.png}
  \caption{Number of sampled examples for the date difference EG for our large size models, and \fone{} score on IIRC$_\textrm{oracle}$ questions that require date difference reasoning. \at{top caption is very small here you can increase the text sizes in the figures}}
  ~\label{fig:analysis-syn-to-real}
\end{figure}

\paragraph{Endowed skills}

\begin{table}
\centering
        \tiny
        \begin{tabular}{lccccc} \toprule
        
        \emph{Question Type}  & \emph{NMN} & \tfive{-} & \rem{-} & \tfive{-} & \rem{-} \\
        & & \emph{Base} & \emph{Base} & \emph{Large} & \emph{Large}  \\ \midrule 
        Date-Compare & 82.6 & 86.4 & 87.5 & 87.6 & \textbf{89.9} \\
        Date-Difference & 75.4 & 19.6 & 78.9 & 45.4 & \textbf{80.4} \\
        Number-Compare & 92.7 & 91.3 & 95.2 & 97.3 & \textbf{98.5} \\
        Extract-Number & 86.1 & 91.8 & 94.9 & 92.1 & \textbf{95.1} \\
        Count & 55.7 & 80.1 & 86.7 & 86.7 & \textbf{89.2} \\
        Extract-Argument & 69.7 & 87.6 & 86.2 & 90.5 & \textbf{92.1} \\
        \bottomrule 
         
        \end{tabular} 
\caption{F$_1$ on a previously suggested split of the DROP dataset to reasoning skills.} 
\label{tab:analysis-endowed-skills}
\end{table}

In order to check which reasoning skills were endowed to our \rem{} models, we use a previously suggested split of the DROP dataset to reasoning skills \cite{Gupta2020Neural}. Table~\ref{tab:analysis-endowed-skills} presents the \fone{} results for our best \rem{} and \tfive{} models on this split, as well as the original \fone{} results from the neural module network (NMN) model used in \newcite{Gupta2020Neural}. When comparing to \tfive{}, we find the set of endowed skills to be diverse, including date and number comparison, number extraction (superlatives), and counting. In addition, our model outperforms the original neural model network on all reasoning skills.

% \begin{itemize}

%     \item IIRC: show generalization templates that weren’t seen during CPT, like (‘how old’)
%     \item DROP QDMR analysis
%     \item Model size analysis: analysis for the delta between base and large models: (a) MMQA - delta in comparison questions decreases (b) DROP analysis for which questions are answered by a large model and not base (c) IIRC delta remains high - date difference reasoning doesn’t increase with size
%     \item Error analysis: show that many of the errors are for reasoning that weren’t seen in CPT
%     \item Counting/arithmetic: show that the model learns small numbers first (memorization)

% \end{itemize}
